LASER: LAtent SpacE Rendering for 2D Visual Localization

We present LASER, an image-based Monte Carlo Localization (MCL) framework for 2D floor maps. LASER introduces the concept of latent space rendering, where 2D pose hypotheses on the floor map are directly rendered into a geometrically-structured latent space by aggregating viewing ray features. Through a tightly coupled rendering codebook scheme, the viewing ray features are dynamically determined at rendering-time based on their geometries (i.e. length, incident-angle), endowing our representation with view-dependent fine-grain variability. Our codebook scheme effectively disentangles feature encoding from rendering, allowing the latent space rendering to run at speeds above 10KHz. Moreover, through metric learning, our geometrically-structured latent space is common to both pose hypotheses and query images with arbitrary field of views. As a result, LASER achieves state-of-the-art performance on large-scale indoor localization datasets (i.e. ZInD and Structured3D) for both panorama and perspective image queries, while significantly outperforming existing learning-based methods in speed.

==> tabels/table_furnishing_and_saliency.tex <==
\begin{tabular}{cccc}
 & \multicolumn{3}{c}{Recall @ 1m (\%)} \\ 
\hline
\multirow{2}{*}{Furnishing} & Panorama~~ & \multicolumn{2}{c}{Persp.~90\textcolor[rgb]{0.102,0.051,0.671}{\textbf{°}}~FoV} \\
 & - & Random & Saliency \\ 
\hline
Empty & 96.23 & 58.40 & 75.19 \\
Simple & 95.82 & 56.92 & 69.12 \\
Full & 95.52 & 55.80 & 64.17 \\
\hline
\end{tabular}
